Seamlessly Unifying Attributes and Items: Conversational Recommendation for Cold-Start Users

Static recommendation methods like collaborative filtering suffer from the inherent limitation of performing real-time personalization for cold-start users. Online recommendation, e.g., multi-armed bandit approach, addresses this limitation by interactively exploring user preference online and pursuing the exploration-exploitation (EE) trade-off. However, existing bandit-based methods model recommendation actions homogeneously. Specifically, they only consider the items as the arms, being incapable of handling the item attributes, which naturally provide interpretable information of user's current demands and can effectively filter out undesired items. In this work, we consider the conversational recommendation for cold-start users, where a system can both ask the attributes from and recommend items to a user interactively. This important scenario was studied in a recent work. However, it employs a hand-crafted function to decide when to ask attributes or make recommendations. Such separate modeling of attributes and items makes the effectiveness of the system highly rely on the choice of the hand-crafted function, thus introducing fragility to the system. To address this limitation, we seamlessly unify attributes and items in the same arm space and achieve their EE trade-offs automatically using the framework of Thompson Sampling. Our Conversational Thompson Sampling (ConTS) model holistically solves all questions in conversational recommendation by choosing the arm with the maximal reward to play. Extensive experiments on three benchmark datasets show that ConTS outperforms the state-of-the-art methods Conversational UCB (ConUCB) and Estimation-Action-Reflection model in both metrics of success rate and average number of conversation turns.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> introduction_bak.tex <==
\section{introduction}
 
%XN (P1): Background of rec, drawback of offline static recom
Recommendation system plays an increasingly important role in the current era of information explosion. In past decades, most recommendation research has been focused on advancing offline predictive models, ranging from traditional collaborative filtering \cite{BPR, fastMF}, content- and context- aware filtering~\cite{ACF, FM}, to the recently prevalent neural network methods~\cite{NCF, cheng2016wide} and graph-based methods~\cite{wang2019neural, ying2018graph}. Such methods learn the static preference of users from past interaction history, which inevitably, suffer from the inherent limitation of performing real-time personalization. User preference is dynamically changing by nature; more challengingly, new users could come anytime, interacting with the system very shortly but expecting to receive desired recommendations. 
 

% XN (P2): Online recom address the cold start scenario, EE tradeoff, drawback of online recom -- no attrbiute
To capture dynamic user preference in real-time, it is essential to explore the unknown preference of a user, and meanwhile to exploit the known preference of the user to meet his past interest. Such exploration-exploitation (EE) trade-off is a core problem in \textit{online recommendation} research and has been intensively studied~\cite{gentile2016context,wu2016contextual,wang2017factorization,wu2018learning,li2010contextual, auer2002finite, murphy2012machine}. A prevalent way is to model it as a multi-armed bandit problem that treats each item as an arm, optimizing the arm selection strategy by interactively recommending items to the user. Although such solution is mathematically well-formulated, we argue that it is very inefficient to explore the whole item space. In many real-world applications, the number of items could be very large-scale, e.g., there are over billions of products (videos) in Alibaba (YouTube). Soliciting user preference in the level of \textit{single item} is far less efficient than that in the level of \textit{item attribute} --- if we know what attributes are preferred by the user now, we can safely filter out the items that do not contain the preferred attributes and increase the learning speed  by a large margin. For example, if a user specifies that he wants to watch \textit{Science Fiction} movie, we can safely ignore other categories of movies. 

% XN (P3): Introduce conversational recsys, Li Hang limitation
A very recent work by \citet{zhang2020toward} is the first to consider asking attributes in online recommendation, naming the new task as \textit{conversational contextual bandit}. They emphasize two challenges in the task: 1) which attributes to ask, and 2) how to build a better bandit model with the attribute feedback, developing a UCB-based method to incorporate attributes as arms. However, another critical problem --- whether should the system ask an attribute or recommend an item in a conversation turn --- is not seriously considered. Specifically, they model attributes and items as two different kinds of arms, and manually define a function to determine the timing of attribute asking (e.g., asking an attribute per three turns). We argue that the strategy of attribute asking is an important factor that affects the effectiveness and usability of a \textit{conversational recommendation system} (CRS), which aims to hit the preferred item(s) with the fewest turns, so as to avoid bothering the user with too many questions. Moreover, they solve the extended bandit problem under the UCB framework, requiring heavy mathematics to derive a near-optimal solution, which makes the method difficult to extend with additional factors for practical use.  

% XN (P4): Our method
In this work, we explore the central theme of conversational recommendation for cold-start users. Besides the typical EE trade-off, our key consideration is to model attributes and items in the same arm space, and develop a holistic solution to solve the three core questions in CRS --- 1) what attributes to ask, 2) what items to recommend, and 3) whether to ask or recommend in a turn --- in a \textbf{seamless} way. To this end, we propose a new \textit{Conversational Thompson Sampling} (CoTS) model, extending the Thompson Sampling framework to build the holistic solution. Specifically, {\color{red} CoTS ... wenqiang: adding sentences on how to extedn TS}. In contrast to ConUCB~\cite{zhang2020toward}, our methods ... {\color{red} advantages over CoTS, fewer maths, easy to extend/generalize}.

% XN (P5): Another line of conversation rec, EAR, CRM
Lastly, it is worth mentioning that another relevant line of research extends traditional offline recommender models (e.g., factorization machine~\cite{FM}) to the conversational setting~\cite{chen2003understanding,lei2020estimation}. Their idea is to score items and attributes with traditional models trained on historical data, and use a reinforcement learning (RL) agent to learn the attribute-asking policy. Their methods, however, do not consider the EE trade-off, which we believe is critical factor for online recommendation especially for cold-start users. Moreover, their methods address each question in CRS with a separate module and glue the multiple modules together, making the overall solution difficult to tune for a new dataset or domain.

% XN (P6): Summary of contribution
The main contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We study the new task of conversational recommendation for cold-start users with attribute preference. By modeling attributes and items as indiscriminate arms in the same space, we propose a holistic solution CoTS to solve the three main questions in CRS in an end-to-end manner. To the best of our knowledge, this is the first time that addresses attribute-aware conversational recommendation with Thompson sampling. 
    \item We construct two datasets from Yelp and lastFM with the simulation of conversations. Extensive experiments show that our CoTS outperforms the state-of-the-art CRS methods ConUCB~\cite{zhang2020toward} and EAR~\cite{lei20estimation} in both metrics of success rate and average turn for cold-start users. Further analyses show the importance of exploration and the effectiveness of CoTS's action policy. All codes and data will be released to facilitate the research community studying CRS.
\end{itemize}

%Having developed for many years, Recommendation Systems already have lots of successful applications. There are various powerful models being well researched ~\cite{fastMF, he2017neural, guo2017deepfm, berg2017graph, chen2017attentive}, most of them utilize historical data to capture user preference. However, the above models do not work well for cold start scenario. Cold start means we'd like to make recommendation for new users with little previous information, which indicates we can not use a large sum of historical interactions to estimate user's preference anymore. To deal with the problem, new recommendation systems which can do online interacting with users have been put forward. The intrinsic objective of these systems is to keep an exploitation-exploration (EE) balance under cold start setting. It means we hope to achieve a good recommendation result for new users in limited interaction turns. This requires the systems both exploit the user's current known interest and explore his new interest to pursue latent larger reward. \\

%经过多年的发展，推荐系统有很多成功的应用。有各种各样powerful的模型被研发出来，他们利用了历史数据capture user preference。但是这些模型对Cold start情况失效了。针对cold start问题，可以online interacting with user的系统被提出来（这里我并不想说online recommendation，要不然开篇就把讨论限制在online recommendation上有点不好，我想突出可以online和user interact，dynamically来估计user preference的系统。这样传统的online recommendation也算，conversational recommendation 也算）。这种系统的本质是 EE balance：(解释EE balance的难点) 要在有限次的interaction当中....

% 为了解决EE问题，online recommendation这个研究分支把整个online recommendation过程model成为一个multi-arm bandit问题，提出了一系列行之有效的解决方法。。。However, the typical setting of the traditional online recommendation systems is keeping recommending items to the user during which a model dynamically update model according to user feedbacks (accept or reject)..在接一句话描述细节。。。尽管取得了阶段性的成功，但是这个模型有一个弱点：只能推不能问，这样一个系统只能模糊地猜测用户喜好。


%To solve EE problem, many works for online recommendation model the whole online recommendation as a muti-arm bandit problem and they put forward a series of methods to solve the problem, such as~\cite{gentile2016context,wu2016contextual,wang2017factorization,wu2018learning,li2010contextual, auer2002finite, murphy2012machine}. However, the typical setting of the traditional online recommendation systems is keeping recommending items to the user during which a model dynamically update model according to user feedbacks (accept or reject). They will tend to recommend the items with known user's preference while exploring user's interest on some other items too. Although these models achieve relative success, there is a weakness among them: the models can only recommend items in each interaction and fail to estimate user's preference in a more efficient way, like asking some questions. This results that the system can only vaguely speculate user's interest by the recommendation results and significantly perform worse than most offline models.
%快速发展的对话技术为解决这个问题带来了希望。他可以用对话dynamically interact with users。。。这样就可以通过问attribute方式更explicitly获取user preference。所以说lihang引入了attribute，但是他的问题是（把item和attribute分来来model了，模型比较碎片化？）
%注：related work中一定要说现在好多对话系统不是在cold start setting下做的。

%Rapidly developed conversational technologies brings hope to deal with the difficulties. By dynamically interacting with users in dialogues, Conversational Recommendations Systems (CRS) can ask user's favoured attributes of the items to explicitly obtain user's preference. This strategy can incredibly decrease the candidate item pool during a conversation, because we only have to consider the items which have the same attributes with those the user has already gives a positive feedback. However, the main difficulty in CRS is to decide when to ask questions and when to recommend items. After all, we can not ask too many questions to make the conversation overly long. Recent works neither trained a policy network on offline dataset Lei et al.~\cite{lei2020estimation} or directly choose a policy function by hand Zhang et al.~\cite{zhang2020toward}. Both of them are not suitable to apply on a complex and dynamic online environment for cold start users.


%In this work, we put forward a new model to do conversational recommendation under cold start scenario, mainly using muti-arm contextual bandit (specifically, Thompson Sampling). Although Zhang et al.~\cite{zhang2020toward} also do contextual bandit in conversational recommendation, they choose a totally hard code policy function for asking and recommending and choose the asked attribute and recommended items by different methods. In contrast, we naturally model all the items and attributes in one space as the equivalent arms in Thompson Sampling and put forward a holistic framework to solve all the four questions in conversational recommendation (when to ask, what to ask, when to recommend, what to recommend), unlike the previous sate-of-art model EARS.~\cite{lei2020estimation} which design several modules to solve these questions separately. In fact, we solve these questions by directly calculate expected rewards of each arm to choice an action to take. What's more, by applying Thompson Sampling to conversational recommendation scenario, our model keeps balance between exploitation and exploration to a great extent, which makes it better to do recommendation under cold start scenario.

%In summary, the main contributions can be concluded as follows:
%\begin{itemize}[leftmargin=*]
%    \item We propose a new scenario of CRS under cold start setting. We then design a model to make use of previous historical information to do initialization for new users and solve EE questions in cold start setting. 
    
%    \item We put forward a holistic framework by modeling all the attributes and items in conversational recommendation as arms to play in muti-arm bandit problem. Benefiting from this, we can apply the methods in bandit to solve the four main questions in CRS mentioned above by simply calculating the expected rewards for each arm. To the best of our knowledge, it is the first time to model all the actions in a whole framework for multi-round conversational recommendation.
    
%    \item To demonstrate the effectiveness of our model, we build two datasets to simulate cold start scenario and do a series of experiments. We show that our model significantly outperforms several existing models on both the success rate and average turn for recommendation. We also design experiments to show both the action choose policy and EE balance strategy contribute a lot to the performance of our model. Besides, we analyse the drawbacks of other models under our setting. All codes and data will be released to assist the further studies on CRS.
    %\item We analyze different settings for CRSs models. To the best of our knowledge, we are the first to discuss those settings.
    %\item We conduct experiment on various settings. We find that, the bigger feature space it is, the significant improvement our model can achieve on both recommendation success rate and dialogue coherence. All codes and data will be released to assist the further studies of this problem.
%\end{itemize}

\begin{figure}[t]
\label{fig:overall}
\begin{minipage}[t]{1\linewidth}
    \includegraphics[width=\linewidth]{CoTS.pdf}
    %\caption{caption1}
    \label{f1}
\end{minipage}%


\caption{The example of CoTS' actions during a whole conversational recommendation process for cold start users. The orange blocks represent operations, green blocks represent parameters and blue blocks resemble agents in the scenario.} 
\vspace{5pt}

\end{figure}


%注：这一段还需要好好地顺一下，把模型的细节和优点能够有机的结合起来。
%为了解决这个问题，本文提出一个更整体的模型。。在thompson sampling的框架下，把item和attribute model到一个空间当中。…..（稍微一两句介绍方法的细节），，
%注：看行文语境，是在intro中还是在abstract中解释我们不用LinUCB。
%比起之前的模型，我们这个方法最大的有点就是整体化，自然地把item和attribute model到同一个空间，利用了TS的框架来来解决 ears提出conversational recommendation的那“四个问题”。。。。unlike SOTA EARS，design各个模块来处理各个问题。。。并且，它利用了TS，也很好地balance了EE，更好地适用于cold start的问题。。






















\endinput

==> introduction_bak_2.tex <==
\section{introduction}
%XN (P1): Background of rec, drawback of offline static recom
Recommendation system plays an increasingly important role in the current era of information explosion. In past decades, most recommendation research has been focused on advancing offline predictive models, ranging from traditional collaborative filtering \cite{BPR, fastMF}, content- and context- aware filtering~\cite{ACF, FM}, to the recently prevalent neural network methods~\cite{NCF, cheng2016wide} and graph-based methods~\cite{wang2019neural, ying2018graph}. Such methods learn the static preference of users from past interaction history, which inevitably, suffer from the inherent limitation of performing real-time personalization. User preference is dynamically changing by nature; more challengingly, new users could come anytime, interacting with the system very shortly but expecting to receive desired recommendations. Conversational recommendation brings a promising solution to directly obtain users' preference and improve the efficiency of recommendation, especially for the cold start users, by utilizing a natural mechanism (i.e., conversation) to interact with and obtain dynamic preferences from the users.
 
{\color{red}Conversational recommendation brings a promising solution to the cold start problems as it brings a natural mechanism (i.e., conversation) to interact with and obtain dynamic preferences from the users. \citet{christakopoulou2016towards} make the first step to introduce conversational recommendation to the cold start problem. They identified the key problem of the cold start conversational recommendation is the Exploration -- Exploitation (EE) trad-off. Therefore, they borrow ideas from multi-arm bandit methods, which is known to be powerful in the EE trad-off problem, to select items to demonstrate to users by modeling each item as an arm. However, the resultant conversational recommendation system can only keep recommending items to the users. We argue that it is very inefficient to explore the whole item space. In many real-world applications, the number of items could be very large-scale, e.g., there are over billions of products (videos) in Alibaba (YouTube). Soliciting user preference in the level of \textit{single item} is far less efficient than that in the level of \textit{item attribute} --- if we know what attributes are preferred by the user now, we can safely filter out the items that do not contain the preferred attributes and increase the learning speed by a large margin. For example, if a user specifies that he wants to watch \textit{Science Fiction} movie, we can safely ignore other categories of movies. 
}

 Nowadays, there are already many applications in industrial field. For example, when users swipe to browse the videos on Kuaishou, the app will sometimes display an interface asking the user to choose his preferred labels. The biggest game platform Steam will provide some estimated preferred labels for the user to click. Besides, many companies,such as YouTube, Spotify, Xiami Music, Xianyu, also combine the strategy of asking attributes into their recommendation system to improve the performance. Considering a real world scenario: the system is asked to recommend videos for users with little or no interaction history. It is usually hard to directly implement some traditional algorithms to make recommendation cause they need much historical data for training process. In this case, asking the user about his preferred attributes of the videos is an effective way to quickly find out his interest. So each time the system can either recommend a set of videos by a specific strategy or display a dialogue box to ask the user' preferred labels for video themes. On the one hand, knowledge about the user's preferred labels can directly help the system narrow down the candidate video pool by overlooking videos without these labels. On the other hand, its main task is still to successfully recommend videos and the user may feel disturbed if the dialogue box is shown too frequently. To deal with that, there are two requirement for the system: 1) decide the strategy of asking and recommending in an intelligent way; 2) keep balance between exploiting current known preference and exploring latent new interest for cold start users to achieve good performance. \\
%To this end, Lihang further develop XXX which considers asking attributes aside from choosing items for recommendations. They model attributes and items into two sets of different items, introduce (disadvantages.)

\begin{figure}
  \centering
  \subfigure[Steam]{
    \label{fig:subfig:a} %% label for first subfigure
    \centering
    \includegraphics[width=1.3in]{Steam.pdf}}
  \hspace{0.5in}
  \subfigure[Kuaishou]{
    \label{fig:subfig:b} %% label for second subfigure
    \centering
    \includegraphics[width=0.8in]{Kuaishou.pdf}}


\caption{The displayed dialogue box in Steam and Kuaishou to ask users choose their preferred labels.} 
\vspace{-0.06cm}
\end{figure}

{\color{red} A very recent work by \citet{zhang2020toward} consider asking attributes in the cold start setting, naming the new task as \textit{conversational contextual bandit}.} They emphasize two challenges in the task: 1) which attributes to ask, and 2) how to build a better bandit model with the attribute feedback, developing a UCB-based method to incorporate attributes as arms. However, another critical problem --- whether should the system ask an attribute or recommend an item in a conversation turn --- is not seriously considered. Specifically, they model attributes and items as two different kinds of arms, and manually define a function to determine the timing of attribute asking (e.g., asking an attribute per three turns). We argue that the strategy of attribute asking is an important factor that affects the effectiveness and usability of a \textit{conversational recommendation system} (CRS), which aims to hit the preferred item(s) with the fewest turns, so as to avoid bothering the user with too many questions. Moreover, they solve the extended bandit problem under the UCB framework, requiring heavy mathematics to derive a near-optimal solution, which makes the method difficult to extend with additional factors for practical use. 


% XN (P4): Our method
In this work, we explore the central theme of conversational recommendation for cold-start users. Besides the typical EE trade-off, our key consideration is to model attributes and items in the same arm space, and develop a holistic solution to solve the three core questions in CRS --- 1) what attributes to ask, 2) what items to recommend, and 3) whether to ask or recommend in a turn --- in a \textbf{seamless} way. To this end, we propose a new \textit{Conversational Sampling} (CoS) model, inspired from the Thompson Sampling framework to build the holistic solution. Specifically, it {\color{blue}xxx... advantages...need to be corresponded to the method part.}.
% Wenqiang: No need to mention LinUCB as we do not doing Thompson Sampling.

% XN (P5): Another line of conversation rec, EAR, CRM
Lastly, it is worth mentioning that another relevant line of research extends traditional offline recommender models (e.g., factorization machine~\cite{FM}) to the conversational setting~\cite{chen2003understanding,lei2020estimation}. Their idea is to score items and attributes with traditional models trained on historical data, and use a reinforcement learning (RL) agent to learn the attribute-asking policy. Their methods, however, do not consider the EE trade-off, which we believe is critical factor for cold-start users. Moreover, their methods address each question in CRS with a separate module and glue the multiple modules together, making the overall solution difficult to tune for a new dataset or domain.

% XN (P6): Summary of contribution
The main contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We study the new task of conversational recommendation for cold-start users with attribute preference. By modeling attributes and items as indiscriminate arms in the same space, we propose a holistic solution CoS to solve the three main questions in CRS in an end-to-end manner. 
    \item We construct two datasets from Yelp and lastFM with the simulation of conversations. Extensive experiments show that our CoTS outperforms the state-of-the-art CRS methods ConUCB~\cite{zhang2020toward} and EAR~\cite{lei20estimation} in both metrics of success rate and average turn for cold-start users. Further analyses show the importance of exploration and the effectiveness of CoS's action policy. All codes and data will be released to facilitate the research community studying CRS.
\end{itemize}

%Having developed for many years, Recommendation Systems already have lots of successful applications. There are various powerful models being well researched ~\cite{fastMF, he2017neural, guo2017deepfm, berg2017graph, chen2017attentive}, most of them utilize historical data to capture user preference. However, the above models do not work well for cold start scenario. Cold start means we'd like to make recommendation for new users with little previous information, which indicates we can not use a large sum of historical interactions to estimate user's preference anymore. To deal with the problem, new recommendation systems which can do online interacting with users have been put forward. The intrinsic objective of these systems is to keep an exploitation-exploration (EE) balance under cold start setting. It means we hope to achieve a good recommendation result for new users in limited interaction turns. This requires the systems both exploit the user's current known interest and explore his new interest to pursue latent larger reward. \\

%经过多年的发展，推荐系统有很多成功的应用。有各种各样powerful的模型被研发出来，他们利用了历史数据capture user preference。但是这些模型对Cold start情况失效了。针对cold start问题，可以online interacting with user的系统被提出来（这里我并不想说online recommendation，要不然开篇就把讨论限制在online recommendation上有点不好，我想突出可以online和user interact，dynamically来估计user preference的系统。这样传统的online recommendation也算，conversational recommendation 也算）。这种系统的本质是 EE balance：(解释EE balance的难点) 要在有限次的interaction当中....

% 为了解决EE问题，online recommendation这个研究分支把整个online recommendation过程model成为一个multi-arm bandit问题，提出了一系列行之有效的解决方法。。。However, the typical setting of the traditional online recommendation systems is keeping recommending items to the user during which a model dynamically update model according to user feedbacks (accept or reject)..在接一句话描述细节。。。尽管取得了阶段性的成功，但是这个模型有一个弱点：只能推不能问，这样一个系统只能模糊地猜测用户喜好。


%To solve EE problem, many works for online recommendation model the whole online recommendation as a muti-arm bandit problem and they put forward a series of methods to solve the problem, such as~\cite{gentile2016context,wu2016contextual,wang2017factorization,wu2018learning,li2010contextual, auer2002finite, murphy2012machine}. However, the typical setting of the traditional online recommendation systems is keeping recommending items to the user during which a model dynamically update model according to user feedbacks (accept or reject). They will tend to recommend the items with known user's preference while exploring user's interest on some other items too. Although these models achieve relative success, there is a weakness among them: the models can only recommend items in each interaction and fail to estimate user's preference in a more efficient way, like asking some questions. This results that the system can only vaguely speculate user's interest by the recommendation results and significantly perform worse than most offline models.
%快速发展的对话技术为解决这个问题带来了希望。他可以用对话dynamically interact with users。。。这样就可以通过问attribute方式更explicitly获取user preference。所以说lihang引入了attribute，但是他的问题是（把item和attribute分来来model了，模型比较碎片化？）
%注：related work中一定要说现在好多对话系统不是在cold start setting下做的。

%Rapidly developed conversational technologies brings hope to deal with the difficulties. By dynamically interacting with users in dialogues, Conversational Recommendations Systems (CRS) can ask user's favoured attributes of the items to explicitly obtain user's preference. This strategy can incredibly decrease the candidate item pool during a conversation, because we only have to consider the items which have the same attributes with those the user has already gives a positive feedback. However, the main difficulty in CRS is to decide when to ask questions and when to recommend items. After all, we can not ask too many questions to make the conversation overly long. Recent works neither trained a policy network on offline dataset Lei et al.~\cite{lei2020estimation} or directly choose a policy function by hand Zhang et al.~\cite{zhang2020toward}. Both of them are not suitable to apply on a complex and dynamic online environment for cold start users.


%In this work, we put forward a new model to do conversational recommendation under cold start scenario, mainly using muti-arm contextual bandit (specifically, Thompson Sampling). Although Zhang et al.~\cite{zhang2020toward} also do contextual bandit in conversational recommendation, they choose a totally hard code policy function for asking and recommending and choose the asked attribute and recommended items by different methods. In contrast, we naturally model all the items and attributes in one space as the equivalent arms in Thompson Sampling and put forward a holistic framework to solve all the four questions in conversational recommendation (when to ask, what to ask, when to recommend, what to recommend), unlike the previous sate-of-art model EARS.~\cite{lei2020estimation} which design several modules to solve these questions separately. In fact, we solve these questions by directly calculate expected rewards of each arm to choice an action to take. What's more, by applying Thompson Sampling to conversational recommendation scenario, our model keeps balance between exploitation and exploration to a great extent, which makes it better to do recommendation under cold start scenario.

%In summary, the main contributions can be concluded as follows:
%\begin{itemize}[leftmargin=*]
%    \item We propose a new scenario of CRS under cold start setting. We then design a model to make use of previous historical information to do initialization for new users and solve EE questions in cold start setting. 
    
%    \item We put forward a holistic framework by modeling all the attributes and items in conversational recommendation as arms to play in muti-arm bandit problem. Benefiting from this, we can apply the methods in bandit to solve the four main questions in CRS mentioned above by simply calculating the expected rewards for each arm. To the best of our knowledge, it is the first time to model all the actions in a whole framework for multi-round conversational recommendation.
    
%    \item To demonstrate the effectiveness of our model, we build two datasets to simulate cold start scenario and do a series of experiments. We show that our model significantly outperforms several existing models on both the success rate and average turn for recommendation. We also design experiments to show both the action choose policy and EE balance strategy contribute a lot to the performance of our model. Besides, we analyse the drawbacks of other models under our setting. All codes and data will be released to assist the further studies on CRS.
    %\item We analyze different settings for CRSs models. To the best of our knowledge, we are the first to discuss those settings.
    %\item We conduct experiment on various settings. We find that, the bigger feature space it is, the significant improvement our model can achieve on both recommendation success rate and dialogue coherence. All codes and data will be released to assist the further studies of this problem.
%\end{itemize}

\begin{figure}[t]
\label{fig:overall}
\begin{minipage}[t]{1\linewidth}
    \includegraphics[width=\linewidth]{CoTS_2.pdf}
    %\caption{caption1}
    \label{f2}
\end{minipage}%

\caption{The example of CoTS' actions during a whole conversational recommendation process for cold start users. Orange blocks represent operations, green blocks represent parameters and blue blocks resemble agents in the scenario.} 
\vspace{3pt}
\end{figure}

\endinput

==> notes.tex <==
\section{Introduction}
out of text citation
~\cite{goker2000personalized}
xxxxx (lei et al., 2020)
xxxx [1]

xxxx~\cite{}

\label{fig:xxxx}
\ref{fig:teaser}

reference
[1] ddddd


in-text-citation
~\citet{goker2000personalized}

Lei et al. (2020) proposed xxxxx
Lei et al. [1] proposed xxxxx

==> references.tex <==
zhang2020toward
zhang2019toward
lei20estimation
rendle2010factorization
he2017neural
guo2017deepfm
berg2017graph
chen2017attentive
gentile2016context
wu2016contextual
wang2017factorization
wu2018learning
li2010contextual

murphy2012machine

graepel2010web
granmo2010solving
may2011simulation

agrawal2013thompson

lai1985asymptotically
chapelle2011empirical
abbasi2011improved
li2016collaborative
wang2016learning
rendle2012bpr  notice to modify the name
christakopoulou2016towards
zhou2011functional
koren2009matrix


berg2017graph
wang2019neural
abernethy2009new
li2015online
nips18/DeepConv,Liao:2018
christakopoulou2018q
zhang2018towards
Sun:2018:CRS:3209978.3210002
priyogi2019preference
liao2019deep
yu2019visual
sardella2019approach
sun2018conversational

==> response.tex <==
Dear Dr Hamed Zamani and Reviewers:

Thank you for your letter and for the reviewers’ comments concerning our manuscript entitled “Seamlessly Unifying Attributes and Items: Conversational Recommendation for Cold-Start Users”. Those comments are all valuable and very helpful for improving our paper. We have studied comments carefully and have tried our best to address all of them in our paper. 


General responses to all reviewers:

Overall, there are two issues needs to be clarified.

First is the cold start setting. We strictly follow the cold start setting but fail to state it clearly. In the revised version, we have re-written Section 5.1.1 to make it clearer. Basically, we partition each dataset into three user-disjoint sets: a training set, a testing set and a validation set. This means that, for any user in one set, we cannot find any corresponding user-item interaction records in the other two sets. To simulate the cold-start setting, we treat the users in the training set as existing users while the users in validation and testing set as new users as their interaction records do not appear in the training set. We first use user-item interactions in the training set to train the embeddings for existing users, items and attribute. Then, for each user in the testing/validation set (i.e., the "new user"), we use one user-item interaction record to simulate one conversation session.
We also notice there might be some misunderstandings on the filtering. We filter out all the USERS (inclusive all their user-item interaction records) with less than 10 records following EAR~\cite{lei20estimation}. This is to make sure we can simulate more than 10 conversations for each user such that our evaluation is more robust. This partition is consistent for all models compared in our experiment, hence should be fair.

Second is the problem formalization of conversational recommendation. Some reviewers believe this work should be more tag-based interactive recommendation instead of conversational recommendation. Actually, in the current problem definition, there are two categorizes of conversational recommendation:  NLP-based and form-based~\cite{abs-2004-00646}. NLP-based setting builds  conversational recommendation as a type a chatbot/dialogue system, which focus more on fluent and diverse dialogue flow, utterance understanding and generation. However, in the form-based setting, users typically follow pre-defined dialogue paths and interact with the application by filling forms or choosing from pre-defined options. Our ConTS belongs to the second category. Inclusive of ours, many recent conversational recommendation systems work also follows the form-based setting such as~\cite{averjanova2008map, hong2010interactive, dietz2019designing, mccarthy2004dynamic}. However, as conversational recommendation is an emerging topic where different researchers define and approach it from different perspective. It is very hard to find a clear cut between the interactive and conversational recommendation. 

Here are detailed responses to each comment:



Reviewer #1:

Comment 1.1: 
The novelty of the motivation of the paper could be improved. It is a natural extension for modeling the cold-start users that follow the multidimensional Gaussian distribution, which is the core motivation in this paper. However, to assume the preference of cold-start users as the average of existing users is more like a general strategy with less novelty for modeling the cold-start users. My concern is that since the datasets have been preprocessed to filter out the user-item interactions. Whether the "existing" users include the filtered interactions or not? If included, I don't believe it's a fair and appropriate comparison since it’s kind of utilizes the external knowledge while other baselines don't. If not, I'm concerned about the motivation since the existing users may not be able to provide the average preference.

Response 1.1: 
We believe there are some important misunderstandings. First, the novelty of this paper is "seamlessly unifying attributes and items in the same space which enables the model to solve the three conversation policy questions in a holistic Thompson Sampling framework". Initializing the preference of cold-start users as the average of existing users’ is only a technical operation to utilize the existing historical information but we do not claim any novelty about it. Other baselines such as Abs greedy~\cite{christakopoulou2016towards} also applies similar strategy do such initialization. 
As for the dataset issue, we apologize to fail to make it clear in the original manuscript and have totally re-written section 5.1.1 in the revised version. The key point has been discussed in the ``general responses to all reviewers". Here, I just provide an additional information. Although the "existing user set" (i.e., the training set) does not contain the filtered user-item interactions, our initialization strategy is also useful because we still have a large number of users in the filtered dataset. Our experiments also validates this: as demonstrated in Section 5.3, the comparison of ConTS and ConTS-${u}_{init}$ validates the usefulness of our initialization. Experiments in Abs Greedy also validates such kind of initialization is useful.


Comment 1.2: 
Compared to ConUCB and EAR settings, which could be regarded as more general CRS, instead of the cold-start users, the contribution of ConTS is limited to the cold-start users. It would be a complete work adding the both quantitative and qualitative analysis of why ConTS may not be compatible for general users.

Response 1.2: 
Yes, this is a good suggestion. Thompson Sampling is originally designed for the cold-start users who has totally no historical records at all. We therefore in the previous version only conduct experiments for such users. In the revised version, we have added section 5.7 to discuss the model performances under different cold-start degrees. We find that although more historical records help Thompson Sampling to get stronger performances, this positive effect is very limited. In contrast, EAR can  better utilize historical records. This suggests that in the real application, it is better to apply ConTS to the users when there are very few historical records. When the records become more, it would be more helpful to shift to warm-start solutions like EAR. 


Comment 1.3: 
TS may not be the stat-of-art method for the arm chosen over the contextual online settings. Compared to the ConUCB, the experimental performance of ConTS is much better. It would be more convincing to include the theoretical analysis compared to ConUCB. Eq 16-20 and table 6 has justified the effectiveness of TS in terms of attributes and item modeling. It is not certain that utilizing TS would gain better UCB for contextual bandit algorithms. Also, the comparison may also take LinUCB into consideration.

Response 1.3: 
Again, we believe there are misunderstandings about the main contributions in this paper. In this paper, our key idea is that "seamlessly unifying attribute and item strategy" is effective. This makes the attribute choosing more intelligent and automatic. Here, we choose Thompson Sampling as the basis to implement this idea because Contextual Thompson Sampling is reported to be more effective than contextual UCB methods~\cite{russo2014learning, osband2017optimistic, chapelle2011empirical}. In addition, we also demonstrate that our Seamless-UCB, the model variant that implements our “seamless strategy” in the framework of UCB, outperforms ConUCB in Section 5.5. The key difference between ConUCB and Seamless-UCB is that ConUCB employs a handcrafted strategy (i.e., the b(*) function) to choose attributes while we use our "seamless strategy" to do so. This further validates our "seamless strategy". 
However, we agree there might be fancy arm choosing algorithms which has better performances, we may extend our frameworks to them. But as the first step, we limit our discussions on classic bandit algorithms.

As for the theoretical analysis, ConUCB only considers the performance related to the turn of recommendation and ignores the cost of asking questions. This is only part of the complete CRS problem hence is not comparable to ours. However, how to conduct the theoretical analysis considering cost of asking questions is still an open problem. We therefore leave it for future works.


Comment 1.4: 
After reviewing the case study, it seems that the users only provide short responses without providing any further detailed instructions or questions to the agent in CRS. I totally agree that users usually show less patience in CRS, but I doubt the proposed online settings over the CRS since it doesn't include any language modeling for conversational semantic understanding. On the other hand, why is it necessary to design the user with four choices of feedback and then to design the corresponding action policy? In real application of CRS, the recommended list could always exist and keep dynamically changing as the conversations move forward. It would be promising for the community to understand the importance of the online settings.

Response 1.4: 
As discussed in the "general response to all reviewers", our setting is form-based conversational recommendation~\cite{abs-2004-00646}. In such setting, the key research question the conversation strategy in pre-defined dialogue paths and dialogue actions. Therefore, all the models conduct conversation through predefined templates. While we do agree that involving more dynamically generate natural languages would be much more interesting, the optimization would be too difficult as the action space has not been defined. 

One issue that we want to clarify is that the form-based conversational recommendation itself has wide applications. A typical example is given in Section 1 of the Kuaishou app (Figure 1 (b)), where the system will pop up a box to ask the user’s favorite categories of videos. When the system decides to ask questions, the box will occupy the screen of user’s phone and there are no more recommended videos to be displayed. After the user chooses his preferred categories, the system will re-rank videos for the user to click and watch.

Reviewer #2:

Comment 2.1: 
In Equation (9), how do you calculate the inverse \Sigma^{-1} for large \Sigma matrices?

Response 2.1: 
we utilize the function np.linalg.inv() in numpy to calculate the inverse matrix.


Comment 2.2: 
A complexity analysis of the proposed model is missing.

Response 2.2:
Thanks for this comment. We have added a new section (i.e., section 4.5) to briefly analyze the complexity of ConTS. The complexity is $O(2*d*(n+k)+d^2)$. Since ConTS is based on contextual Thompson Sampling, the detailed analysis of complexity of ConTS is the same as contextual Thompson Sampling. Therefore, we directly give the result as readers can easily find the detailed analysis on the classic papers about contextual Thompson Sampling~\cite{li2010contextual, agrawal2013thompson}.

Comment 2.3: 
This paper targets to combat the issue of cold-start users in conversational systems. However, cold-start users are not properly defined in the experiments, as described in the last paragraph of Section 5.1. In related work, cold-start users are defined as the users with less interactions. Why did not you use a binning strategy based on users’ interactions, to split users into different cold-start degrees, for example, users<5 interactions, users 5-10 interaction and so on. Furthermore, the results should be reported for different cold-start degrees to show that indeed the proposed model can face the cold-start problem.

Response 2.3: 
This is a good suggestion. We have conducted additional experiments and added one section (i.e., Section 5.7) to discuss the performance of ConTS in different cold-start degrees. The results are shown in Figure 4. When there are very few existing historical records, ConTS consistently gets better performances on both Average Turn and SR@15. As the existing records become more, the performance of EAR increases much sharper than ConTS and eventually outperforms ConTS by a large margin. This suggests that in the real application, it is better to apply ConTS to the users when there are very few historical records. When the records become more, it would be more helpful to shift to warm start solutions like EAR.



Comment 2.4: 
What hyper-parameter tuning strategy did use in your experiments? Did you split the datasets into training, validation and test sets?

Response 2.4: 

We have added this detail in Section 5.2.4. Specifically, we tune the parameters on the validation set. The values of user's feedback in ConTS is searched in the range of [-8, 8] and we apply grid search to find the optimal settings. We find that the absolute value of positive feedback should be larger while the absolute value of negative feedback should be smaller for better performance. We partition the user-item interactions of each dataset into the ratio 7:1.5:1.5 for training, validation and testing. More details about the data splitting are given in Section 5.1.1.



Comment 2.5: 
What is the parameter setting for ConUCB?

Response 2.5: 
We detailly introduce the parameter setting for ConUCB in Section 5.2. Specifically, all the parameters are tuned following the methods in original paper. The optimal performance can be achieved when \lambda\mathrm{=0.8} and \widetilde{\lambda}\mathrm{=1}. We also explore different policy functions in ConUCB and report the best result, which is discussed in details in Section 5.4.


Comment 2.6: 
In section 5.2.3 SR@t should be formally defined e.g., in Equation.

Response 2.6: 
We have given the equation of SR@t in Section 5.2.3. Specifically, it is defined as the ratio of conversations which successfully make recommendation using at most t turns. The equation is SR@t=\frac{#\ successful\ conversations\ by\ turn\ t}{#\ conversations}.


Comment 2.7: 
The language could be improved, there are syntax errors or informal sentences.

Response 2.7: 
we are very grateful to Reviewer for reviewing the paper so carefully. We have corrected all the syntax errors list here. We tried our best to improve the manuscript in terms of languages.






Reviewer #3:

Comment 3.1: the paper is actually an interactive recommendation paper rather than a conversational recommendation paper because items and attributes are considered as homogeneous entities to the policy network, as a result, even though attributes are described as questions, they are actually no difference in terms of the interactive filtering.

Response 3.1: 
As described in the "general responses to all reviewers", this work falls in the scope of form-based conversational recommendation system. In the form-based conversational recommendation system, users typically follow pre-defined dialogue paths and interact with the application by filling forms or choosing from pre-defined options. 
Comparing to interactive filtering, there do existing many differences in term of the problem setting. The main difference is the way of using attributes. In term of the problem setting, asking attribute and recommending items are actually heterogeneous.  Asking attributes can help to obtain user’s preference and make a successfully recommendation in the future, while recommending user’s preferred items can directly successfully end the conversation. However, in terms of our solution, we try to adopt the idea of treating items and attributes homogeneous in terms of modeling. Intuitively, this work can be viewed as "discussion homogeneous solution for the heterogeneous problem". But in the problem setting, we still treat it as a form-based conversational recommendation.



Comment 3.2: Although the authors claimed it works on cold-start recommendation, the experimental setting is actually very far-away from cold-start setting in terms of two important perspectives. First, users with less than 10 view records and attributes with less than 5 occurrences are filtered out. Second, the construction of training and testing sets is also very tricky -- they sample users until the accumulated click histories of the sampled users take up to 70\% of the user-item interaction records, this means that the remaining 30\% users, which are taken as testing users, are actually not cold-start users, these users are identical with the 70\% training users in terms of interaction history. The experimental setting must be corrected to reflect a truly cold-start recommendation scenario.

Response 3.2: 
There are important misunderstandings. We apologize for the unclear writing in our previous version and have totally re-written section 5.1.1 in the revised version. The response has been summarized in the  ``general response to all reviewers". Key points are: 1) The training, validation and testing sets are user-disjoint. In the online testing stage, we use one user-item interaction record in the testing set to simulate a dialogue session. For the testing users, there are no corresponding user-item interaction records in the training set. From this perspective, we call our setting as cold-start. 
As for filtering, this is to make sure we can simulate more than 10 conversations for each user such that our evaluation is more robust.


Comment 3.3: 
How to define and calculate SR@t is not very clear. Does it mean success rate *at exactly* turn t or success rate *with at most* t turns? Authors said successful rate *by* turn t, so seems to be the second case. Table 3 also seem to be the second case (by setting max turn 15). However, Figure 3 seems to be the first case, since the lines are not monotonically increasing. The meaning of SR@t should be clear and consistent throughout the paper.

Response 3.3: 
Here *by* means *at most* and is consistent throughout the paper. We rewrite the definition of SR@t in Section 5.2.3. Specifically, SR@t is defined as  SR@t=\frac{#\ successful\ conversations\ by\ turn\ t}{#\ conversations}. The reason why the lines in Figure 3 are not monotonically increasing is that the index of y-axis is Success Rate* instead of SR@t. We have defined Success Rate* in the caption of the figure. Success Rate* denotes the diﬀerence of SR@t between each method and the system represented by the line of y\ =\ 0. For example, we set ConUCB as y=0 on LastFM and SR@15 of ConUCB and ConTS is 0.446 and 0.756 respectively. Therefore, the Success Rate* of ConTS at turn 15 should be 0.310 (0.756-0.446).
We use Success Rate* in the Figure to facilitate visualization of comparison for different models.

Comment 3.4: The case study in Figure 4 is unclear and cherry-picking. To make it more clear, authors would better show what is the ground truth video the user liked, what are the features of the ground truth video, and what items are recommended. Besides, all cases result in one round of recommendation with correct items, even the EAR case where no asked attribute is correct. Finally, authors only show the case that supports their claims. It's better and necessary to also show some bad cases. Having bad cases is fine, every model has bad cases, and they help readers to better understand the model. But hiding the bad cases is not fine.

Response 3.4: Thanks for your comments. We have rewritten this section to flesh it out. First, we detailed the features and content of the video the user like and try to give more analyses. Besides, we tried to demonstrate the recommended 10 items in each round but felt it too redundant. Instead, we have uploaded the real interaction logs of those cases as supplementary materials and we will also provide such materials to public once this paper got accepted. Finally, we have added more cases to discuss the property and advantages of other baselines like EAR and ConUCB. We find that ConUCB might be better when the user's interest is hard to infer. And if the new user has similar preference with the average of existing users', EAR can be more efficient to quickly acquire his interest and successfully end the conversation.


-------------------------------------------------------------------------------


We have tried our best to improve the manuscript and made some changes in the manuscript. These changes will not influence the content and framework of the paper.

We appreciate for Editors/Reviewers’ warm work earnestly, and hope that the correction will meet with approval. Once again, thank you very much for your comments and suggestions.

Sincerely, 
Shijun Li, Wenqiang Lei, Qingyun Wu, Xiangnan He, Peng Jiang and Tat-Seng Chua


